Physical Property Understanding from Language-Embedded Feature Fields

Can computers perceive the physical properties of objects solely through vision? Research in cognitive science and vision science has shown that humans excel at identifying materials and estimating their physical properties based purely on visual appearance. In this paper, we present a novel approach for dense prediction of the physical properties of objects using a collection of images. Inspired by how humans reason about physics through vision, we leverage large language models to propose candidate materials for each object. We then construct a language-embedded point cloud and estimate the physical properties of each 3D point using a zero-shot kernel regression approach. Our method is accurate, annotation-free, and applicable to any object in the open world. Experiments demonstrate the effectiveness of the proposed approach in various physical property reasoning tasks, such as estimating the mass of common objects, as well as other properties like friction and hardness.

==> fig/failure_cases.tex <==
\begin{table*}[!t]
    \centering
    \resizebox{\linewidth}{!}{
\setlength{\tabcolsep}{0.2em} %
\renewcommand{\arraystretch}{1.}
    \begin{tabular}{ccccc}
    \tiny{RGB} &
   \tiny{Material Prediction} &
   ~~~~~~~ & 
    \tiny{RGB} &
    \tiny{Material Prediction }
    \\
   
        \includegraphics[height=1.5cm]{fig/failure_cases/lamp1.jpg}  &
        \includegraphics[height=1.5cm]{fig/failure_cases/lamp_failure_pcd.png}  &
         &
        \includegraphics[height=1.5cm]{fig/failure_cases/bed1.jpg} 
        &
         \includegraphics[height=1.5cm]{fig/failure_cases/bed_failure_pcd.png}
         \\
         
        \tiny{GT Mass: 1.7 kg} &
   \tiny{Pred Mass: 30.1 kg} &
   ~~~~~~~  & 
    \tiny{GT Mass: 39.9 kg} &
   \tiny{Pred Mass: 435.1 kg} 
    \end{tabular}

    }
    
    \includegraphics[width=\linewidth, trim={0.5cm 0 0 0}, clip]{fig/failure_cases/mat_legend_supp.png}
    
\captionof{figure}{\textbf{Example failure cases.} In order to show the geometry of the objects' bounding volumes, the model predictions are visualized as point clouds where each point is a voxel center from the bounding volume. Errors in the geometry (such as the filled in lamp shade) and errors in the CLIP-based retrieval both contribute to incorrect mass predictions.}
\label{fig:failure_cases}
\end{table*}
